Towards an Effective Organization-Wide Bulk Email System

Bulk email is widely used in organizations to communicate messages to employees. It is an important tool in making employees aware of policies, events, leadership updates, etc. However, in large organizations, the problem of overwhelming communication is widespread. Ineffective organizational bulk emails waste employees' time and organizations' money, and cause a lack of awareness or compliance with organizations' missions and priorities. This thesis focuses on improving organizational bulk email systems by 1) conducting qualitative research to understand different stakeholders; 2) conducting field studies to evaluate personalization's effects on getting employees to read bulk messages; 3) designing tools to support communicators in evaluating bulk emails. We performed these studies at the University of Minnesota, interviewing 25 employees (both senders and recipients), and including 317 participants in total. We found that the university's current bulk email system is ineffective as only 22% of the information communicated was retained by employees. To encourage employees to read high-level information, we implemented a multi-stakeholder personalization framework that mixed important-to-organization messages with employee-preferred messages and improved the studied bulk email's recognition rate by 20%. On the sender side, we iteratively designed a prototype of a bulk email evaluation platform. In field evaluation, we found bulk emails' message-level performance helped communicators in designing bulk emails. We collected eye-tracking data and developed a neural network technique to estimate how much time each message is being read using recipients' interactions with browsers only, which improved the estimation accuracy to 73%. In summary, this work sheds light on how to design organizational bulk email systems that communicate effectively and respect different stakeholders' value.

==> analysis.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% oscillation_analysis.tex: Analysis of Neutrino Oscillations:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Analysis}
\label{analysis_chapter}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Analysis Procedure {{{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Analysis Procedure}
\label{anaproc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Analysis Result {{{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Analysis Result}
\label{neymanana}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%}}}


==> backup/study3_backup.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% data_set.tex:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Evaluation Tools for Better Transparency and Targeting \cite{evaluation}}
\label{study3}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








% Ahn et al. \cite{ahn2003design} posed three questions for the designers to consider when designing CRM platforms. Except that ``What form must we use the data in?'' is more related to the technical implementation of databases, we could see that the platforms for organizational bulk emails should be different from the platforms for external bulk emails in chapter 2 in terms of these two questions:
% \begin{itemize}
%     \item What is the purpose of data analysis? The purpose of data analysis in organizational bulk emails is to optimize the whole organization's benefits, while the purpose of analyzing external bulk emails is to optimize the bulk email senders' benefits. The current CRM platforms' costs analysis focuses on the sender-side, but the costs for organizational bulk emails also include the employees and the organization's time and money.
    
%     \item What data must we prepare? The current bulk email platforms' targeting and personalization mostly depend on the demographics (e.g., age, location, department, job code) and users' interactions with the websites. However, within organizations, whether a message should be sent to an employee depends on both the employee's preferences and their job responsibilities, which their job codes and departments could not fully represent. 

% \end{itemize}

% I would like to design a test tool for organizational bulk emails. This tool would mainly be a web application that enables communicators to send test emails, collect employees' behavior data and feedback, and visualize bulk emails' performance and costs. It is aimed to help communicators understand:

% \begin{enumerate}
%     \item Which employee groups might find this email interesting/work-relevant --- the estimated performance (e.g., open rates, interest rates/open rates/work-relevance rates/click rates) of different employee groups.
%     \item  The estimated costs (e.g., reading time, money costs) of different employee groups.
%     \item The feedback from employees on the bulk emails' designs/contents.
% \end{enumerate}

\section{Introduction}
Organizations often send bulk emails to communicate policy updates, event notifications, and organizational plans to their employees. We call such bulk emails sent from an organization to its employees as \textbf{organizational bulk emails}. Organizations send these bulk emails via customer relationship management (CRM) platforms like Salesforce and Mailchimp, which provide metrics like the open rate of emails and click rate of URLs \cite{bernstein2015research, monitor2012campaign}. However, open rate and click rate might not be enough to support \textbf{communicators} (organizations' employees in charge of designing and sending organizational bulk emails) in making editing / targeting decisions on bulk emails. Open rate can be an overestimation of employees' awareness because employees often open and close bulk emails in a few seconds and skip their contents. Many organizational bulk emails focus on letting employees be aware of information instead of clicking links \cite{kong2021learning}. And within organizations, we also need to evaluate bulk emails' time cost to recipients (employees) as organizations pay for their time on reading emails and maintain communication channels' reputation \footnote{In this paper, we use ``channel'' to refer to a series of bulk communications / newsletters with the same sender identity (the FROM field) and brand (in the title or format, e.g., xxx Brief Dec 1, 2022).}. Therefore we would like to learn how communicators currently evaluate organizational bulk emails, identify design opportunities, and build an evaluation platform that better supports them in understanding their audience and designing bulk emails. We posed the following research questions:

\noindent\textbf{RQ1} What are communicators' current practices of evaluating bulk emails and expectations regarding CommTool (the bulk email evaluation platform we would design)?

\noindent\textbf{RQ2:} How do recipients interact with CommTool?

\noindent\textbf{RQ3:} What are communicators' experiences with CommTool? 

\noindent\textbf{RQ4:} How does email impact its channel's reputation?




We conducted interviews, iterative designs \cite{zimmerman2014research}, and field tests to study these questions. We started with expert interviews (5 communicators of the studied university) to learn about their experiences and practices with evaluating organizational bulk emails. We found that besides open rate and click rate, communicators need various metrics to make decisions, like the \textbf{message-level} performance \footnote{``Message'' here refers to single stories / pieces of information in bulk emails.} and bulk emails' cost and impact on channel reputation. 
The requirement specifications of bulk email evaluation platforms were then summarized from the qualitative analysis of these interviews' transcripts. Then a bulk email evaluation platform (CommTool) was designed iteratively through 7 usability tests. To evaluate the platform, we then conducted a 2-month field test in the studied university with 5 communicators and 149 recipients (employees of the university). The evaluation of CommTool was based on: 1) the log data of the communicators and recipients; 2) the survey responses of the communicators collected through the field test; 3) interviews with the communicators after the field test.

Compared to the previous studies which evaluated bulk communication \cite{kraut2005pricing, reeves2008marketplace} based on some heuristics (e.g., 1 cent per email), CommTool provided message-level performance and cost based on real measurements of reading time, relevance rate, skip / skim / read-in-detail rate. CommTool also estimated emails' impact on their channels' reputation, given their performance collected during the field test. 

Communicators reflected that CommTool helped them better understand their audience via message-level awareness information such as reading time, custom feedback such as comments, and group-level interest information. They also suggested improvements in features around cost and reputation estimation. Specifically, the cost metrics did not influence the organization leaders' decisions on sending messages out, and communicators preferred to observe trends themselves instead of seeing a ``reputation'' value. We concluded with design suggestions based on the feedback we received. The rest of the paper includes related work, formative study, field study, and discussion.




\section{Related Work}
As we discussed in Chapter \ref{related_work_chapter}, one challenge of organizational communication is employees' information overload --- employees’ perceptions that they receive more information than they can handle effectively \cite{10.1145/1180875.1180941}.
\citeauthor{davenport2001attention} proposed that employees have an ``attention budget'' --- more information they receive from the information, more information would be ignored \cite{davenport2001attention}. \citeauthor{vsliburyte2004internal} proposed that in evaluating the effectiveness of organizational communication, the stakeholders' \textbf{cost} (e.g, time cost) needs to be considered \cite{vsliburyte2004internal}. For example, \citeauthor{jackson2001cost} monitored 15 employees' laptops and found they need 6 seconds to decide whether to open an email and 64 seconds to recover from an email interruption on average \cite{jackson2001cost}. \citeauthor{10.1145/1180875.1180941} conducted a nationwide organization survey and found that email volume is positively correlated with the feeling of email overload at work \cite{10.1145/1180875.1180941}. Given these challenges regarding the effectiveness of organizational bulk emails, many organizations take action (see below) to evaluate their bulk emails' performance.

As reviewed in Chapter \ref{related_work_chapter}, many large business platforms are supporting bulk email senders in evaluating their emails' performance, such as Salesforce, Mailchimp, Revue, Constant Contact, etc \cite{bernstein2015research, monitor2012campaign}. The evaluation features supported by these platforms include the open rates, click rates, number of subscriptions and their trends, A/B Tests, etc.

Besides the business CRM platforms, several marketing studies also shed light on how to evaluate bulk emails (though most of them focused on bulk emails to external customers). \textbf{``Awareness and impact''} of bulk emails are the two concepts that often mentioned. \citeauthor{cruz2008evaluating} interviewed CRM users and learned that reaching and awareness (e.g., knowing the brand) is more important than behavioral metrics (e.g., hits and clicks) in evaluating marketing emails \cite{cruz2008evaluating}. \citeauthor{morgan2012developing} reviewed the metrics of the current CRM platforms and pointed out that they focused on what can be measured quickly (e.g., open rate of marketing emails) instead of what should be measured (e.g., changes in the perceptions of the brand) \cite{morgan2012developing}. \citeauthor{todor2016marketing} strengthened the importance of understanding bulk emails' consequence \cite{todor2016marketing}, like the return of interest, the number of businesses generated, etc. \citeauthor{siano2011exploring} proposed a framework for senders to measure their reputation --- recipient's perception of a specific sender's communication quality \cite{siano2011exploring}. In the engineering field, there is work focusing on the API design and database integration of CRM platforms \cite{stubarev2018development, xu2015infrastructure}.

We noticed a lack of HCI work on designing evaluation platforms for organizational bulk emails. Their design requirements might be different from the commercial CRM platforms (which focus on external marketing emails). For example, organizations pay for employees' time on reading bulk emails; organizational bulk emails might focus less on conversion rate / return of interest but more on awareness of organizational goals. In this study, we would like to understand organization communicators'  experience with evaluation platforms, specify requirements, and design platforms to better support communicators in designing bulk emails.

In the following, we introduce a formative study for the iterative design process of CommTool (RQ1), and a field test for evaluating CommTool (RQ2 --- 4).

\section{Formative Study (RQ1)}
We first conducted formative studies to 1) understand communicators' current practice of evaluating bulk emails; 2) identify design requirements; 3) deploy CommTool iteratively. Our study site is a public university with over 25,000 employees and several campuses. We collaborated with the communicators of its central units (e.g., presidential offices), who are in charge of organizing, designing, and distributing university-wide bulk emails to all staff / faculty. This study is approved by the IRB of <blinded>. 




\subsection{Expert Interviews}
We first conducted expert interviews with 5 university communicators to learn RQ1. We applied an artifact-walkthrough approach  \cite{beyer1999contextual} by which we asked about communicators' practices with specific email cases. During each interview, the communicator selected 5 emails they sent out recently, then answered the following questions:
\begin{itemize}
    \item Communication Goal: Did you come up with the content by yourself, or did your clients provide it? Who are you hoping to reach? How do you hope they react to these messages? What open rate/action rate would you be happy with? How much employee time would be taken according to your estimation?

    \item Communication Practice: How did you decide the ways of writing the content? How did you send it (e.g., in a newsletter, separate email, or distribution channels)? How did you evaluate the effectiveness?
    
    \item Expectations of Evaluation Platforms: Which information do you hope to have when you evaluate this email? Any challenges you have met with the current evaluation platform?
\end{itemize}

In the end, we introduced several design ideas for the evaluation platform CommTool, and asked the communicators their preferences on these ideas and the reasons.

We interviewed via zoom, and each interview took around 60 minutes. We recruited through the university's communicator forum. The forum director identified a list of potential participants working in the central communication offices. We contacted 6 communicators, and 5 (C1 to C5) agreed to participate in this expert interview.

For data analysis, the first author conducted the initial open coding of the first interview. The research team met weekly to discuss whether enough repeated themes emerged and whether more interviews were needed. Requirement specifications were summarized with the affinity diagramming approach \cite{holtzblatt1997contextual}. We summarized our findings around RQ1 below.

\noindent\textbf{Observation 1: Communicators design / send / evaluate bulk emails for their clients.} 

Communicators sent those bulk emails for their clients within the university, such as their managers, university leaders, and central offices. They need to communicate with their clients first if they want to make some changes to bulk emails based on the evaluation results. For example, C2 described this editing process:
\begin{quote}
\textit{``So how it usually works is they (the clients) will have an email, and I'll review that and take that information to draft an email. And then they'll approve it, and then I'll send ... Especially when it comes to newsletters where there are multiple parties, it would be helpful to say: you know, based on the research that we've done on this newsletter you know, this kind of content doesn't isn't is appealing to this audience, so we're not going to include it.'' (C2)}
\end{quote}
Therefore, a bulk email evaluation platform can change the status quo of designing bulk emails only if the platform supports communicators to reach an agreement with their clients on the design. Based on this observation, we proposed the following requirement:

\noindent Requirement 1: The evaluation platform should enable communicators to share the results and communicate with their clients.

\noindent\textbf{Observation 2: The metrics provided by the current platforms are not enough in measuring awareness and relevance.}

Communicators noticed that their open rate looks pretty good --- usually above 60\%. But on another side, employees might not pay enough attention to their emails. For example, C1 talked about an email sent to over 8100 faculty:

\begin{quote}
    \textit{``There's an open rate of 62\%. It might count as an open rate if they just tap it in their inbox before archiving it. So I'm not sure if that means people actually put their eyes on it, or just like cleared it out.'' (C1)}
\end{quote}

C3 talked about an email asking all employees to check their Human Resource dashboard, but employees seem to pay less attention to it: 

\begin{quote}
    \textit{``So it (the email about checking HR dashboard) has a high open rate, 80\%, but only 10\% of the audience that even got to that dashboard to see that data. It (the email) probably doesn't give them enough information to know if they've needed to pay attention, and we don't have enough information to know if those people are paying attention.'' (C3)}
\end{quote}

In summary, there is a gap between the current performance metrics to how well the employees are aware of those bulk emails' contents and how they perceive the relevance of those emails. Based on this observation, we proposed the following requirement:

\noindent Requirement 2: The evaluation platforms should provide metrics around awareness and relevance besides open rate and click rate.

Besides that, since each bulk email often contains multiple messages, the realization of these requirements implies that the granularity of those metrics should not only be limited to per email but also per message:

\noindent Requirement 3: The evaluation platform should provide both email-level and message-level metrics.

\noindent\textbf{Observation 3: Communicators sometimes need feedback in custom formats.}

Besides metrics in fixed formats, communicators also mentioned various formats of feedback they would like to have. The examples mentioned by communicators include whether the recipients already knew the contents, whether the recipients were busy when receiving those emails, the job codes of the recipients who found those emails relevant, the recipients' devices, etc.

\begin{quote}
    \textit{``We've (the communication unit) had discussions about like what time of day people want to receive emails, is it first thing in the morning, or are they overwhelmed by first thing in the morning.'' (C4)}
\end{quote}

\begin{quote}
    \textit{``The challenge we have for employee benefits, for example, and some other communications is really about which job codes are relevant, for example, some of the vaccine requirement information for specific employee groups.'' (C3)}
\end{quote}

Based on this observation, we proposed the following requirement:

\noindent Requirement 4: The evaluation platform should enable communicators to collect custom feedback.

\noindent\textbf{Observation 4: Communicators need employee group's interest to better target messages.}

Communicators mentioned that, especially for communications sent to a large group, their audience is too mixed that communicators do not know which employees might be interested in which messages. And if they have such interest information of different employee groups, they might be able to better target the messages. For example, C2 talked about this challenge when they are sending communications widely:

\begin{quote}
    \textit{``It's hard to know when you're kind of trying to send to a large group of people, a bunch of different stuff --- you don't always know what it is they want to see, or what they're really interested in. If there is some way to fine-tune it (the newsletter) to opportunities, information, news, and stories that different people are really interested in, that would be helpful.''}(C2)
\end{quote}

Therefore we proposed the following requirement:

\noindent Requirement 5: The evaluation platform should enable communicators to understand different employee group's interests.


\noindent\textbf{Observation 5: Communicators realize that bulk email has impacts but cannot measure them.}

Communicators understood that bulk email might bring costs, such as money for paying employees' time, or impact the channel's reputation. They also thought that showing costs to their clients might help in persuading their clients to remove some contents (though they also expressed concerns about to how much extent the cost data could influence their clients). Currently, communicators do not have access to such costs on the current bulk email evaluation platform. For example, C2 talked about how they perceived the potential use of cost data:

\begin{quote}
    \textit{``We don't know, how much time people spend on email and how much money the university loses --- if some people (clients) are very driven by data, and that can help. But when you're working with somebody who just really wants, who really thinks whatever they have to say are important to their to the audience, I don't know if that is going to help.'' (C2)}
\end{quote}

C5 mentioned that their audience stopped reading emails from some channels, and they used other channels instead.
\begin{quote}
    \textit{``We found that if it's like a director of undergraduate studies that's sending out a survey, having it in that professor's name will increase opens tremendously rather than just from the department which people stop reading.'' (C5)}
\end{quote}

With these observations, we proposed the following requirement:

\noindent Requirement 6: The evaluation platform should provide communicators with the impact of bulk communication (e.g., money / reputation cost).

As the communicators mentioned, we are uncertain about to how much extent the clients would take these cost data into consideration, and we would like to observe that during the field test.

\noindent\textbf{Observation 6: The evaluation platform should be light-weight.}

Communicators mentioned that a challenge of getting deep evaluation results for them is that the process is complicated, and they are also overwhelmed by daily work.

\begin{quote}
    \textit{``The current way of doing (deep evaluation) is focus group (usability lab). It is expensive, ineffective, and it's a challenge for us that we have no such internal service on feedback sessions.'' (C3)}
\end{quote}

Therefore, a bulk email evaluation platform should match the following requirement:

\noindent Requirement 7: The platform should be lightweight --- it should take no significant effort for communicators to evaluate bulk emails deeply beyond getting their main job done.

\subsection{Iterative Design}
Based on the requirements above, an initial version of CommTool was deployed and tested by the research team. After the research team reached an agreement on the usability of the platform, we invited communicators to conduct a 30-min usability test. The usability test aims to understand CommTool's workflow's intuitiveness and its metrics' clarity.

During the usability tests, the communicators were asked to explore the platform and complete the following tasks: 1) create a channel and send an email from that channel; 2) find the performance reports of those emails and tell us how they interpret those metrics; 3) share the reports with their clients. The value of the metrics was simulated during the usability tests. We observed whether they met any difficulties in completing the tasks, and whether they understood the metric reports. We then revised the platform according to their feedback. We stopped inviting communicators when the newly invited communicator used the platform smoothly without guidance. We conducted 7 usability tests in the end. We made the following changes to CommTool during the usability tests:


\noindent\textbf{Visibility of Comment Area. }Communicators would like the platform to be more communicator-focused. One point that raises concern is that the recipients who commented might naturally be more disgruntled, or have more negative things to say. Based on that, the comment area is changed to only fully accessible to the corresponding communicator, and the recipients would not be able to see each others' comments (except comments from senders).

\noindent\textbf{Definition of Reading Time / Read Rate / Detail Rate. } Communicators indicate that they would like the reading time calculation to exclude the recipients who did not open the emails, because they already got that information from the open rate. But for the calculation of the read rate and the read-in-detail rate, they prefer to consider all the recipients; then they intuitively can compare the open rate, read rate, and read-in-detail rate together and use them to measure the recipients' awareness.

\noindent\textbf{Provide Definition Tips of Metrics. }As CommTool provides various metrics, communicators cannot remember how we define each metric and ask for explanations during the usability tests. Therefore we provided tip buttons next to each metric in the reports to give detailed definitions. The definitions of the metric we used are summarized as below:




\subsection{Design of CommTool.}
\noindent\textbf{Workflow:} CommTool's workflow (Figure \ref{fig:workflow}) is similar to the workflow of the university's current bulk email evaluation platform (Salesforce). In step 1, communicators upload emails to CommTool, preview them, and send them to recipients (our study participants). The recipients receive emails with the same title, sender name, and personalized links in their inboxes (step 2). The personalized links enable recipients to open these links on any device without login into CommTool, while we can record their data (step 3). Then CommTool collects data from recipients and summarizes metric reports. Communicators would be able to check metric reports in real-time, and also (step 4). After 24 hours (to give recipients enough time to react), communicator gets a reminder email to check reports and fill in research surveys (step 5). 

\begin{figure}[!htbp]
\centering
  \includegraphics[width=1\columnwidth]{study3_folder/workflow.png}
  \caption{Communicator's workflow of evaluating organizational bulk emails through CommTool.}~\label{fig:workflow}
\end{figure}
\begin{table}[!htbp]
\centering
\caption{Metric Definitions.  Email-level metrics are shown in the email dashboard. Message-level metrics are shown in the message dashboards and report dashboards.}~\label{tab: metric_def}
\arrayrulecolor[rgb]{0.753,0.753,0.753}
\scalebox{0.7}{
\begin{tabular}{!{\color{black}\vrule}l|l!{\color{black}\vrule}l|l!{\color{black}\vrule}} 
\arrayrulecolor{black}\hline
\multicolumn{2}{!{\color{black}\vrule}c!{\color{black}\vrule}}{\textbf{Email-Level Metrics }}                                                                                                                                                                                                                                                   & \multicolumn{2}{c!{\color{black}\vrule}}{\textbf{Message-Level Metrics.}}                                                                                                                                                                                          \\ 
\arrayrulecolor[rgb]{0.753,0.753,0.753}\hline
\begin{tabular}[c]{@{}l@{}}Click\\Rate\end{tabular}        & \begin{tabular}[c]{@{}l@{}}The percentage of the implicit recipients who \\at least clicked one link in this email.\end{tabular}                                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Click\\Rate\end{tabular}         & \begin{tabular}[c]{@{}l@{}}The percentage of the implicit recipients\\who at least clicked one link in this message.\end{tabular}                                                                  \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Read\\Rate\end{tabular}         & \begin{tabular}[c]{@{}l@{}}The percentage of the implicit recipients who \\at least skimmed one message of this email or \\read it in detail.\end{tabular}                                                                                                                       & \begin{tabular}[c]{@{}l@{}}Read\\Rate\end{tabular}          & \begin{tabular}[c]{@{}l@{}}The percentage of implicit recipients who\\skimmed this message or read it in detail.\end{tabular}                                                                      \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Detail\\Rate\end{tabular}       & \begin{tabular}[c]{@{}l@{}}The percentage of the implicit recipients who \\at least read one message of this email in detail.\end{tabular}                                                                                                                                       & \begin{tabular}[c]{@{}l@{}}Detail\\Rate\end{tabular}        & \begin{tabular}[c]{@{}l@{}}The percentage of the implicit recipients\\who read this message in detail.\end{tabular}                                                                                \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Reading\\Time\end{tabular}      & \begin{tabular}[c]{@{}l@{}}The average number of seconds the implicit \\recipients who opened this email spent \\reading this email.\end{tabular}                                                                                                                                & \begin{tabular}[c]{@{}l@{}}Reading\\Time\end{tabular}       & \begin{tabular}[c]{@{}l@{}}The average number of seconds the implicit\\recipients who opened this email spent\\reading this message.\end{tabular}                                                  \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Estimated\\Cost\end{tabular}    & \begin{tabular}[c]{@{}l@{}}The estimated money cost of this email: the \\average reading time * open rate * \$40 hour rate\\* the actual number of recipients of this newsletter. \\6 seconds are added for each recipient's time on\\making read / unread decisions.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Estimated\\Cost\end{tabular}     & \begin{tabular}[c]{@{}l@{}}The estimated money cost of this message:\\the average reading time * open rate * \$40\\hour rate * the actual number of recipients.\end{tabular}                         \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Relevance\\Rate\end{tabular}    & \begin{tabular}[c]{@{}l@{}}The percentage of the explicit recipients who at\\least indicated one message of this email that is\\relevant to them.\end{tabular}                                                                                                                   & \begin{tabular}[c]{@{}l@{}}Relevance\\Rate\end{tabular}     & \begin{tabular}[c]{@{}l@{}}The percentage of the explicit recipients\\who indicated that this message is relevant.\end{tabular}                                                                    \\ 
\hline
\# Comments                                                & \begin{tabular}[c]{@{}l@{}}The number of comments the explicit recipients \\left on this email.\end{tabular}                                                                                                                                                                     & \# Comments                                                 & \begin{tabular}[c]{@{}l@{}}The average number of seconds the implicit\\recipients who opened this email spent\\reading this message.\end{tabular}                                                  \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Open\\Rate\end{tabular}         & \begin{tabular}[c]{@{}l@{}}The percentage of the implicit recipients who \\opened this email.\end{tabular}                                                                                                                                                                       & \begin{tabular}[c]{@{}l@{}}Who are\\Interested\end{tabular} & \begin{tabular}[c]{@{}l@{}}The percentage of different categories\\(departments, job categories) of recipients\\who are interested (clicked/read/indicated\\relevant) in this message.\end{tabular}  \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Reputation\\Change\end{tabular} & \begin{tabular}[c]{@{}l@{}}This email's influence on this newsletter's reputation:\\this newsletter's predicted future open rate - this \\email's open rate.\end{tabular}                                                                                                          & \multicolumn{1}{l}{}                                        &                                                                                                                                                                                                      \\
\arrayrulecolor{black}\hline
\end{tabular}
}
\end{table}

\noindent\textbf{Requirement 3, message-level metrics:} For clarity, we first introduce our designs for requirement 3 --- providing both email-level and metric-level metrics to communicators. In CommTool, when communicators upload an html email, the email would be automatically split into sections in preview (by recognizing html tags like <h2>, <h3>, etc.), as displayed in Figure \ref{fig:message_level}. And given the html length of each message, CommTool recognizes whether each section is just a title (like the ``TOP NEWS'' in Figure \ref{fig:message_level}) or is a message with contents (like the ``An apple a day ... '' in Figure \ref{fig:message_level}). Then CommTool adds surveys under those messages --- ``survey'' here means we would collect metrics for these messages. CommTool also enables communicators to remove / add / merge sections, and add / remove surveys in case the split is incorrect. 


\begin{table}
\begin{minipage}{.48\textwidth}

\centering
  \includegraphics[width=1\columnwidth]{study3_folder/message_level.png}
  \captionof{figure}{CommTool can automatically split an html email into single messages during editing.}~\label{fig:message_level}

\end{minipage}%
\hspace{0.05in}
\begin{minipage}{.46\textwidth}
\centering
  \includegraphics[width=1\columnwidth]{study3_folder/explicit_implicit.png}
  \captionof{figure}{The email received by implicit recipients is just like the original email. The email received by explicit recipients would include ``relevant-to-me'' buttons and comment areas.}~\label{fig:explicit_implicit}
\end{minipage}%
% \vspace{-0.1in}
\end{table}

\noindent\textbf{Requirement 2 \& 6, awareness / impact / relevance metrics:} CommTool supports communicators in collecting the awareness / impact / relevance metrics on both message level and email level. For awareness, we calculate the recipients' open rate for each email, average reading time, read (skim or read-in-detail) rate, and read-in-detail rate of each email / message. For impact, we calculate the esimated cost of each email/message and each email's estimated impact on its channel's reputation. For relevance, we calculate the percentage of recipients who viewed an email/message as relevant (either work-relevant or personally interesting) to them, or clicked them. The definitions of metrics are summarized in Table \ref{tab: metric_def}. In the dashboard of email's performance and dashboard of message's performance (see Figure \ref{fig:dashboard}), communicators would be able to see the metrics above in real-time (and they will receive a reminder email to check these metrics after 24 hours of sending the email).



An important step in calculating these metrics is that CommTool splits the recipients into an implicit recipient group and an explicit recipient group. The implicit recipients were asked to react to the emails they received as normally as they could --- CommTool uses their log data to calculate the open rate, reading time, read rate, read-in-detail rate, click rate, and estimated cost. The explicit recipients were asked to read those emails and indicate whether each message was relevant to them and leave comments under the messages if applicable. We split the recipients into these two groups because ``indicating relevance'' and ``commenting'' are time-consuming and ask for more attention from the recipients. We do not want these actions to interfere with the calculation of awareness metrics. 

Specifically, for email-level reading time, CommTool use the average time the implicit recipients are active on the email page \footnote{``Active'' here means that the window is visible, and if there are no interactions (scroll / click / mouse hover) in the past minute a window will pop up to check whether recipients would like to stay on the page.}. 6 seconds are added for each recipient's time on making read / unread decisions, based on \cite{jackson2001cost}'s finding that 70\% of emails were opened within 6 seconds in the workplace. For message-level reading time, CommTool estimated a recipient's reading time of each message based on their interactions with the emails' pages (e.g., scroll, click, mouse hover) and behavioral patterns (e.g., scroll / click frequency). The ground-truth data (reading time of each message) and features (recipients' interactions and patterns) were collected through eye-tracking tests with Tobii Pro eye-tracker. In those tests, we recorded 9 university employees reading university bulk emails through CommTool. We collected 1 data point on whether a message was being read or not for each message per second, employees' interactions with webpages, resulting in a 200k dataset. The final model (a two-tower neural network model) reaches a 27\% percentage error on reading time in the 9-fold test split by recipients' data \cite{eyetrack}. The read (skim or read-in-detail) rate and read-in-detail rate are calculated given the number of words of each message / email and their reading time, whether a message / email was skipped / skimmed / read-in-detail by a recipient is separated by the reading speed 400 words / min and 200 words / min (400/60 words and 200/60 words per second). These limits were selected based on a comprehension level of 70\%, and 80\% in \cite{nocera2018rapid}.



% \begin{itemize}
%     \item Relevance rate: a message's relevance rate is the percentage of explicit recipients who clicked the relevant-to-me button in Figure \ref{fig:explicit_implicit}; an email's relevance rate is the percentage of explicit recipients that at least indicated one message in the email as relevant.
%     \item Click rate: a message's click rate is the percentage of implicit recipients who clicked the hyperlinks in it; an email's click rate is the percentage of explicit recipients that at least clicked one message in the email.
%     \item Open rate: the percentage of implicit recipients who clicked the personalized links they received (Step 2, Figure \ref{fig:workflow}).
%     \item Reading time: for email, we use the average time the implicit recipients are active on the email page \footenote{''Active'' here means that the window is visible, and if there are no interactions (scroll / click / mouse hover) in the past minute a window will pop up to check whether participants would like to stay on the page.}. For message, CommTool estimated a recipient's reading time of each message based on their interactions with the emails' pages (e.g., scroll, click, mouse hover) and behavioral patterns (e.g., scroll / click frequency). The ground-truth data (reading time of each message) and features (recipients' interactions and patterns) were collected through eye-tracking tests with Tobii Pro eye-tracker. In those tests, we recorded 9 university employees reading university bulk emails through CommTool. We collected 1 data point on whether a message was being read or not for each message per second, employees' interactions with webpages, resulting in a 200k dataset. The final model (a two-tower neural network model) reaches a 26\% percentage error on reading time in the 9-fold test split by recipients' data (see anonymized citation attached \cite{eyetracking}).
%     \item Read (skim or read-in-detail) rate and read-in-detail rate: given the number of words of each message / email and their reading time, whether a message / email was skipped / skimmed / read-in-detail by a recipient is separated by the reading speed 400 words / min and 200 words / min (400/60 words and 200/60 words per second). These limits were selected based on a comprehension level 70\% and 80\% in \cite{nocera2018rapid}.
%     \item Estimated (money) cost: calculated based on reading time + 6 seconds interruption time for deciding to open the email or not (based on \cite{jackson2001cost}'s finding that 70\% of emails were opened within 6 seconds in the workplace), the actual size of the corresponding venue's mailing list, and the average hourly rate of employees of the study site (\$40/hour). 
%     \item Impact on venue reputation: we defined each email's impact on its venue's reputation as the predicted open rate of the next email - the open rate of the current email. Based on the performance data of each email collected during the field test, we built a logistic model by which we use the open rate, reading time, click rate, read rate, read-in-detail rate, \# comments, relevance rate, history open rate to predict the next email's open rate from that venue. We started showing this ``reputation change'' metric in week 3 of the field test and updated the model weekly.
% \end{itemize}


\begin{figure}[!htbp]
\centering
  \includegraphics[width=0.9\columnwidth]{study3_folder/dashboard.png}
  \caption{The email/message dashboards of CommTool. The message dashboard (top) shows message-level metrics. The email dashboard (bottom) shows email-level metrics. }~\label{fig:dashboard}
\end{figure}

\noindent\textbf{Requirement 5, different employee group's interest:} On the dashboard page which shows the sample email (Figure \ref{fig:group_interest}), when communicators click ``Who are interested?'', a detailed view of different unit/job's interest rate will be shown. ``Interested'' here is defined as either an implicit recipient clicked / read a message or an explicit recipient indicating that the message is relevant.

\begin{figure}[!htbp]
\centering
  \includegraphics[width=0.6\columnwidth]{study3_folder/group_interest.png}
  \caption{The report dashboard of a sample email. Communicators would be able to see the number of implicit recipients who clicked the message's hyperlinks / the number of implicit recipients, the number of explicit recipients who viewed it as relevant / the number of explicit recipients, average reading time, estimated cost, and the interest rate split by unit / job categories.}~\label{fig:group_interest}
\end{figure}



\noindent\textbf{Requirement 4, custom feedback:} CommTool also enables communicators to collect custom feedback. Communicators can add their questions in the comment area (e.g., ``Would you like to attend this program'' in Figure \ref{fig:message_level}). Communicators' questions would be pinned in the comment area and highlighted by ``from sender'' (anonymously). Explicit recipients would see these pinned questions and answer them anonymously if they would like to (see Figure \ref{fig:share}).



\noindent\textbf{Requirement 1, share with clients:} CommTool enables communicators to share the results with their clients. On each dashboard (message performance, email performance, recipient view), there is a ``share'' button, communicators can click this button, add high-level summaries to that dashboard, and get the shareable links (see Figure \ref{fig:share}). Their clients do not need to register in CommTool to view these reports but can also post comments as the senders of that email with the shareable links.

\begin{figure}[!htbp]
\centering
  \includegraphics[width=0.9\columnwidth]{study3_folder/share.png}
  \caption{Share Report. Communicators can summarize the report in notes and share that link with their clients. Their clients can comment as senders with shareable links.}~\label{fig:share}
\end{figure}

\noindent\textbf{Requirement 7, light-weight use experience:} The whole workflow of evaluation (see Figure \ref{fig:workflow} only needs communicators to copy and paste their email to CommTool, click send, then they will receive results --- in the usability tests, this process took less than few minutes.\\







\section{Field Test (RQ 2---4)}
To evaluate CommTool's usefulness, we conducted a 2-month field test with 5 communicators and 149 recipients (employees of the university).
\subsection{Methods}
The participating communicators were recruited from the communicators we contacted in the expert interviews and usability tests from the central communication offices. Before the field test, we asked each communicator to select a university-wide bulk email channel (sent at least monthly) to participate in the test. Before the field test, we asked the communicators in the past month, on average, how many times they communicated with their clients or shortened content during editing that channel.

The recipients were recruited through 1) the  communicators putting the recruitment message on the selected channels; 2) other mailing lists of the university; 3) the research team distributing the study posters to 38 buildings' poster boards and offices; 4) the university's slack channels. We recruited 149 recipients in total. We split the recipients into explicit/implicit groups randomly (the recipients would stay in the assigned group throughout the whole study) and gave corresponding instructions (see 3.3). Then we gave the communicators the list of recipients to be excluded from the channels during the field test (to avoid these recipients receiving duplicate emails).

During the field test, each time when the communicators sent an email under the selected channel, they would go to CommTool to send the same one to the list of recipients. We logged the recipients' interactions with each email. At the first 9 a.m. after 24 hours after they sent out each email, CommTool will send the communicators a reminder email, asking them to check the reports of that email and answer the research surveys \footnote{The communicators asked for a regular time of receiving reports.}. The research surveys contained 3 questions: 1) Which of these metrics we show on this page help you make future editing / sending decisions? 2) Which editing/sending decisions have you made / will make based on this report? 3) Why are certain metrics helpful/unhelpful to you? Could you give an example of the editing / sending decisions you made based on this report? We also logged whether the communicators read each report, how much time they spent reading, and whether they shared the reports with their clients. 

After the field test, we conducted 30-min interviews with the communicators, with the following questions: 1) What’s your general experience with CommTool? What's its pros and cons compared to your current evaluation platforms? 2) Which features of CommTool do you find helpful / useless? Why? 3) Which decisions do you usually make based on the reports (could you give a specific example)? How do you perceive the cost and performance tradeoff of these emails? 4) Do you have any other features you would like to see in such a bulk email evaluation tool? Would you like to keep using CommTool in the future? Why? The interviews were analyzed following the same practice of expert interviews.

\subsection{Recipients' Interaction with CommTool (RQ2)}

Figure \ref{fig:summary} shows the statistics of recipients' interactions with per email. The level of open rate of each channel is close to their original level (around 70\% for Brief, 60 \% for Communication Blog, 50 \% for Controller's Office, and Research is a brand new channel). 

Most emails were skimmed. Recipients who opened these emails spent around 60 seconds reading long channels like (Brief, Research, and Controller's Office) and around 10 seconds reading the short channel (Communication Blog). The email read rates (of at least reading one message in that email) were below 70\%, and the detail rates were below 60\%. Besides Brief, the relevance rates were below 40\%, and the comment rates were mostly below 10\%.

Recipients were paying less attention over time. Some of them gradually stopped opening emails as channels' open rates decreased by over 10\%. The read rate and detail rate of these channels also decreased through the field test with a scale of 10\% to 30\%, with increasing read speeds. The click rate did not change much through the field test. The relevance rates were decreased by over 20\%, and comment rates were also decreased by over 10\%. These results show that the channels' reputation needs to be protected.


\begin{figure}[!htbp]
\centering
  \includegraphics[width=0.8\columnwidth]{study3_folder/summary.png}
  \caption{Summary statistics of recipients' reactions with each email in different channel. Time refers to the n-th email sent in that channel. Read speed is defined as n\_word / log(1+reading time).}~\label{fig:summary}
\end{figure}


Recipients' comments could be categorized into 3 topics: the reasons that they feel the corresponding messages are interesting / uninteresting personally; how the messages are work-relevant to them; feedback on the content / designs.

\noindent\textbf{Why a message is interesting / uninteresting to me personally: } employees told the senders about why they feel a message is interesting / uninteresting to themselves. The first reason is that the employees have some / no similar experience with the message topic. For example, an employee found a message about Alzheimer research interesting because \textit{``My father-in-law has Alzheimer's so this is very relevant to my personal life.''} An employee found a staff story from another campus uninteresting because \textit{``Don't have a connection to that campus.''}

% The second reason for a message being interesting is that the employees agree with the views in the corresponding messages. For example, an employee found a message about Neuroplasticity in aging interesting because \textit{``In my personal life I also try to focus on holistic well-being in a way that my future self will benefit so this is insightful.''}

The second reason for a message being interesting is that the employees like to see that the university is paying attention to the corresponding topics. For example, an employee is glad to see a message about first-generation student celebration because \textit{``It's helpful to have visibility into central <university name> focuses on first generation students.''}

\noindent\textbf{Why a message is work-relevant to me: } employees tell the sender when they feel a message work-relevant to them. The work-relevance when mentioned on 2 cases: 1) the message is directly related to the employee's job: \textit{``I find virtual events here that I attend for education hours as required by my Dept's Flexible Work Agreement''}; 2) the employee know someone in their units would be relevant: \textit{``This is professionally relevant to me because the unit I work in has polar explorers.''}  (the message is discussing climate-related studies)

\noindent\textbf{Feedback on the content / design: } Recipients give suggestions on the specific content they want to know / how they feel the content could be designed better. For example, an employee suggested \textit{``It would be good to provide more information regarding HOW to set suppliers up with electronic payments - even if it is just "have the supplier contact us directly via phone (\#) or email (address).''} under a message about special check handling. Another employee commented on a long message \textit{``A lot of text with less bold/bullet/other ways to highlight. I would not have made it through the whole thing.''}



\subsection{Communicators' Experience with CommTool (RQ3)}
In this section, we reported when does CommTool help / cannot help communicators in evaluating bulk emails. In the below, Communication Blog's communicator is P1; Brief's communicator is P2; Controller's Office's communicator is P3; Research's 2 communicators are P4 and P5.

\subsubsection{Overall Experience}~\\
\noindent\textbf{Number of times of reading reports}: 22 emails were sent during the study. 5 communicators (<university name> Research has 2 communicators) visited the platforms' dashboards 122 times. The email dashboards were visited 40 times and shared with clients 4 times; message dashboards were visited 53 times and shared with clients 7 times; and detailed report dashboards were visited 29 times and shared 2 times (see Table \ref{tab:summary}). 


\begin{table}[!htbp]
\centering
\caption{Summary Metrics of Communicators' Feedback. The percentages show the rates that the metrics were selected as useful by the communicators in the surveys (averaged by all the channels' statistics).}~\label{tab:summary}
\arrayrulecolor{black}
\scalebox{0.75}{
\begin{tabular}{|ll|ll|ll|} 
\hline
\textbf{Email Dashboard}                                                             &                                                                                  & \textbf{Message Dashboard}                                                             &                                                                                  & \textbf{Report Dashboard}                                                            &                                                                                   \\
\begin{tabular}[c]{@{}l@{}}Total time of email\\dashboards being read\end{tabular}   & 40                                                                               & \begin{tabular}[c]{@{}l@{}}Total time of message\\dashboards being read\end{tabular}   & 53                                                                               & \begin{tabular}[c]{@{}l@{}}Total time of report\\dashboards being read\end{tabular}  & 29                                                                                \\
\begin{tabular}[c]{@{}l@{}}Total time of email \\dashboards being shared\end{tabular}  & 4                                                                                & \begin{tabular}[c]{@{}l@{}}Total time of message \\dashboards being shared\end{tabular}  & 7                                                                                & \begin{tabular}[c]{@{}l@{}}Total time of report \\dashboards being shared\end{tabular} & 2                                                                                 \\ 
\arrayrulecolor[rgb]{0.502,0.502,0.502}\hline
\begin{tabular}[c]{@{}l@{}}\textbf{Email Dashboard}\\\textbf{Metrics}\end{tabular}   & \begin{tabular}[c]{@{}l@{}}\textbf{\% selected}\\\textbf{as useful}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Message Dashboard}\\\textbf{Metrics}\end{tabular}   & \begin{tabular}[c]{@{}l@{}}\textbf{\% selected}\\\textbf{as useful}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Report Dashboard}\\\textbf{Metrics}\end{tabular}  & \begin{tabular}[c]{@{}l@{}}\textbf{\% selected}\\\textbf{as useful}\end{tabular}  \\
Click Rate                                                                           & 48\%                                                                             & Click Rate                                                                             & 57\%                                                                             & Comments                                                                             & 35\%                                                                              \\
Relevance Rate                                                                       & 44\%                                                                             & Read Rate                                                                              & 51\%                                                                             & Relevance Rate                                                                       & 24\%                                                                              \\
Open Rate                                                                            & 33\%                                                                             & \begin{tabular}[c]{@{}l@{}}Average performance \\of all communicators\end{tabular}     & 46\%                                                                             & Who are interested?                                                                  & 15\%                                                                              \\
\begin{tabular}[c]{@{}l@{}}Average performance \\of all communicators\end{tabular}   & 30\%                                                                             & Relevance Rate                                                                         & 38\%                                                                             & Reading Time                                                                         & 8\%                                                                               \\
Read Rate                                                                            & 23\%                                                                             & Reading Time                                                                           & 35\%                                                                             & Click Rate                                                                           & 4\%                                                                               \\
Detail Rate                                                                          & 18\%                                                                             & Detail Rate                                                                            & 15\%                                                                             & Est Cost                                                                             & 0\%                                                                               \\
Reading Time                                                                         & 15\%                                                                             & \# Comments                                                                            & 12\%                                                                             & None of those are helpful.                                                           & 0\%                                                                               \\
\# Comments                                                                          & 12\%                                                                             & Est Cost                                                                               & 11\%                                                                             &                                                                                      &                                                                                   \\
Reputation Change                                                                    & 11\%                                                                             & None of those are helpful.                                                             & 0\%                                                                              &                                                                                      &                                                                                   \\
Est Cost                                                                             & 4\%                                                                              &                                                                                        &                                                                                  &                                                                                      &                                                                                   \\
None of those are helpful.                                                           & 0\%                                                                              &                                                                                        &                                                                                  &                                                                                      &                                                                                   \\ 
\hline
\begin{tabular}[c]{@{}l@{}}\textbf{Email Dashboard}\\\textbf{Decisions}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{\% taken}\\\textbf{this action}\end{tabular}  & \begin{tabular}[c]{@{}l@{}}\textbf{Message Dashboard}\\\textbf{Decisions}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{\% taken}\\\textbf{this action}\end{tabular}  & \begin{tabular}[c]{@{}l@{}}\textbf{Report Dashboard}\\\textbf{Actions}\end{tabular}  & \begin{tabular}[c]{@{}l@{}}\textbf{\% taken}\\\textbf{this action}\end{tabular}   \\
Add more contents                                                                    & 27\%                                                                             & Add more contents                                                                      & 36\%                                                                             & Add more contents                                                                    & 24\%                                                                              \\
None of those                                                                        & 21\%                                                                             & \begin{tabular}[c]{@{}l@{}}Share this report \\with my clients\end{tabular}            & 29\%                                                                             & \begin{tabular}[c]{@{}l@{}}Remove or shorten\\some contents\end{tabular}             & 17\%                                                                              \\
\begin{tabular}[c]{@{}l@{}}Remove or shorten \\some contents\end{tabular}            & 17\%                                                                             & \begin{tabular}[c]{@{}l@{}}Remove or shorten\\some contents\end{tabular}               & 25\%                                                                             & Send to more people                                                                  & 7\%                                                                               \\
\begin{tabular}[c]{@{}l@{}}Share this report \\with my clients\end{tabular}          & 15\%                                                                             & None of those                                                                          & 25\%                                                                             & \begin{tabular}[c]{@{}l@{}}Share this report\\with my clients\end{tabular}           & 7\%                                                                               \\
Send to more people                                                                  & 12\%                                                                             & Send to more people                                                                    & 16\%                                                                             & None of those                                                                        & 7\%                                                                               \\
Send to fewer people                                                                 & 12\%                                                                             & \begin{tabular}[c]{@{}l@{}}Move some contents\\to other newsletter\end{tabular}        & 13\%                                                                             & Send to fewer people                                                                 & 4\%                                                                               \\
\begin{tabular}[c]{@{}l@{}}Move some contents\\to other newsletter\end{tabular}      & 8\%                                                                              & Send to fewer people                                                                   & 8\%                                                                              & \begin{tabular}[c]{@{}l@{}}Move some contents\\to other newsletter\end{tabular}      & 0\%                                                                               \\
\arrayrulecolor{black}\hline
\end{tabular}
}
\end{table}


\noindent\textbf{Ease of use}: In interviews, communicators reflect that the platform is lightweight as they only spent 5 to 10 minutes initiating an evaluation on CommTool: 

\textit{``Everything about the tool, the basics, way things flow, the way you do. Things all seem logical and very useful. (P3)''} 

Communicators are generally satisfied with the readability of dashboards: \textit{``This is a nice overview for quick scanning. (P5)''} 

P1 felt that the designs of the 3 dashboards were too similar, but the reminder email sent to them after 24 hours provided a quick channel to check and differentiate the dashboards: 

\textit{``I'm glad for the email the next morning that links to all 3 of those dashboards, because I don't know if I'd be able to figure out, because the first in the second dashboard looks so similar.'' (P1)}



\noindent\textbf{Compare with existing platform Salesforce}: Communicators feel that Salesforce provides more help in editing email templates, but CommTool provides more information in evaluating emails: 

\textit{``Salesforce has templates which everybody loves. It  has a glamorous interface. CommTool is simpler. It had metrics that people should care about and should be able to track, and at some point, some senior leader is going to ask them for them.  I think it is helpful, especially for people who didn't have a lot of experience with their audience or who were working with completely unknown audiences. (P3)''} 

P1 mentioned that CommTool provided a channel to retrieve various data legally from employees: 

\textit{``Apple messed things up last year. They pull out the tracking pixel before it gets to your inbox --- so the open rates were wrong. In CommTool, people are those who agreed to share this information.'' (P1)}

\noindent\textbf{Sharing reports:} Communicators shared the message dashboards 7 times and shared the email dashboards 4 times. These dashboards provided communicators with the reason for removing/extending specific messages. The per-message reading time specifically gets clients' attention: 

\textit{``Because they are interested in how long people took to read it. They've always had the number of eyes on the open rates. They didn't know that that existed before I started working with them, so they were like, we can tell how many people read the message. Yes? you can. so now they're all comparing numbers with each other, our message did this. They want to go further with metrics like that, how long people are engaged with the content, what their feedback is, and so forth.'' (P3)}


The detailed report page was shared less because clients care more about numbers: \textit{``When I'm talking with the people, they've all seen the message. They've helped write the message in most instances. So they're passed that part, and they want to see the numbers. Plus everyone I work with is a person they're all accountants. So when they see words and pictures, it freaks out a little bit, but when they see numbers they're like. Oh, I love it.'' (P3)}~\\

\subsubsection{Experience with Specific Features}~\\
\noindent\textbf{Message - level versus email - level metrics}  (requirement 3). 
Message metric dashboards were visited more times (53 visits) compared to email metric dashboards (40 visits), see Table \ref{tab:summary}. P2 mentioned that the message dashboard \textit{``is useful if you wanted some more detailed analysis of your readership.''} The report dashboards were visited less (29 visits) --- P2 reflected that communicators who run large newsletters are too busy to look at the details on the report dashboard \textit{``I would not have time to go through all those comments, especially on a list that's 20,000 strong. ''}

\noindent\textbf{Awareness vs relevance vs cost vs reputation metrics (requirement 2, 6)}.
The relevance metric was selected as useful most times, and the awareness metric followed. The cost and reputation metrics were less likely to be used.

Specifically, the email click rate is most usually to be selected as useful (48\% of times) and followed by the relevance rate (44\%). P2 told us that after seeing the email relevance rate, they took more time to  \textit{``consider relevance for audience members when developing content.''}.


Besides, the message-level reading time and read rate are also often found to be helpful. In interviews, P3 said that: 

\textit{``I pay attention to how much time they spent on it when that's available. That is the part of this tool that most interested me. So I could see, Did they engage with the content? And did they spend some time there?'' (P3)} 

Communicators care less about detail rate because most messages only ask people to have some sense of the content: 

\textit{``In-depth reading doesn't really matter much just because it's (the email content) a summary. They (the recipients) can take action based on the email, click in or read the full article.'' (P1)} 

The finance newsletter cares more about read-in-detail rate because they are sending important information that every employee should know: 

\textit{``I'm more interested in the detail than the I mean. All the tools will give you how many eyes looked at it? Right? I want to know how long they spent on it. You know, the University's budget is between 3 and 4 billion dollars a year. It's a lot of money, and most of it is spent on human costs, you know salaries and etc. Every employee should want to care, and the fact that person felt that it wasn't relevant to them meant that they didn't connect with the institution as an entity that has to watch its money, and watch how we behave with it.'' (P3)}

Communicators do trust CommTool's estimation on per-message reading time: 

\textit{``From what I could tell, and I had my own team members look at the email and sort of track. How long it took them to read the sections carefully, and I compared the 2 and I. It seemed very accurate, based on their experience.'' (P2)} 

\textit{``The top article in the top section has about a minute the one spent on it, and then the number gets kind of small as you go down, which makes sense to me because some of these things are meant to scan and other things. It's like you only have this much time to get those attention. So if they spend the most of their attention on the top thing, and then scroll the rest. That seems reasonable.'' (P4)} 


Communicators did review estimated cost but found it less helpful because of the organization's structure: 

\textit{``(We) discussed estimated cost, and while interesting, it didn’t seem to influence leaders' decision to send.'' (P5)} 

Also as we just discussed above, communicators felt some cost does make sense given the value of the information:

\textit{``It (the cost) was frightening. So now, every time I send out an email, I'm like, how much are we actually costing by making people read this? Then I remember we don't send out fluff, or like party invitations, or come to our sale we're sending out. You have work to do. This is related to your work. So we would incur that cost.'' (P3)}

Communicators did not look at the reputation metrics directly but checked out the trend of metrics themselves and had their own judgments:

\textit{``I think it would be most effective in looking at trends over time.'' (P1)} 

\textit{``I'm going to have to see the metrics over time before I make any decisions about changing up the newsletter.'' (P2)} 

\textit{``I did look at the like week to week or message to message on my own like improvement, and if that went up a little bit, I was happy. If it went down, figure out what was in my content that made it go down. I like the predicted reputation change, although I'd want to know how it's actually calculated. But in really simple terms.'' (P3)}

Communicators looked at the average performance of other communicators but did not use it to make decisions --- they preferred to make decisions based on their own data: 

\textit{``I knew there was a total average. I knew my messages were probably different than other messages, so I didn't pay attention to comparing them very much.'' (P1)}





\noindent\textbf{Custom feedback} (requirement 4). Comments gave communicators direct help with writing and formatting (see 4.2 for employees' comments). P3 indicates that based on the comments they received, they would like to make the content clear: \textit{``We've removed a layer of formality from our messaging. We try to be brief, be bright. Taxes shouldn't be scary.'' (P3)}

We also notice that bi-directional communication gets more feedback than single-direction communication. In our study, an email that the communicator has back-and-forth conversations with recipients gets 107 comments while the others are below 40. Some communicators did not use this feature because they did not notice this feature and said that they would reply:

\textit{``If they're (recipients) asking a direct comment like a direct question. (P1)''} 

P3, who got much feedback, gave us suggestions on how to get more replies: 

\textit{``If you ask them unexpected questions, or you ask them in a less formal way, they're more likely to respond. So I think that's why I got a lot of comments.'' (P3)}


\noindent\textbf{Group-level interest} (requirement 5). P4 and P5 from the research newsletter particularly look at ``who are interested'' to ``Consider relevance/interest for audience members and which audiences respond to the types of messages when developing content''. But they felt that the ``who are interested'' feature could be more useful if they could setup groups themselves: 

\textit{``Whenever you have that level of detail, it's interesting. I'm seeing all these different colleges. And that's great. But it's not maybe necessarily useful for us to know that. For us, it would be interesting to see the breakdown between staff and students and faculty.'' (P4)}.

These findings suggest that 1) current bulk email evaluation platforms, besides open / click rate, should take more active actions on collecting the relevance data (like by adding a small relevance to me button under each email), skim-level awareness, and trend of metrics; 2) the evaluation platform should allow message-level custom feedback, and especially encourage the bi-direction communication between senders and recipients; 3) if we want to control bulk emails' time cost, we need to build the mechanism that can influence organization leaders.




\subsection{Email's Impact on Reputation (RQ4)}
In this section, we reported our results around RQ4: email's impact on its channel's reputation. We defined reputation's change as $reputation_t = open\_rate_{t+1} - open\_rate_t$ (the difference between an email sent at time $t$'s open rate to its next open rate). We run ordinary least square models (with constant) between $reputation_t$ and each $metric_t$. The coefficients' values, p-values (for the hypothesis $coefficient \neq 0$), and confidence intervals are reported in Table \ref{tab: coef}.

We found click rate positively correlated with reputation change (coef=0.221, p-val=0.049). Though none of the reading time, read rate, or detail rate correlated with reputation change, the ratio between click rate to read rate is positively correlated with reputation change (coef=0.169, p-val=0.026). This result matches the intuition --- the emails that interest the recipients who read them can build up their reputation. Interestingly, the comment rate was negatively correlated with reputation change (coef=-0.260, p-val=0.041*). According to the contents of the comments we received, a potential explanation is that most recipients only commented when they found an email irrelevant or confusing (about contents, designs, intentions, etc.); therefore, these recipients are less likely to open the next email.




\begin{table}[!htbp]
\centering
\caption{Coefficients between email's performance with its reputation's change. CI: the [0.025,0.975] confidence interval of the corresponding coefficients.}~\label{tab: coef}
\arrayrulecolor[rgb]{0.8,0.8,0.8}
\scalebox{0.7}{
\begin{tabular}{!{\color{black}\vrule}c|c|c!{\color{black}\vrule}c|c|c!{\color{black}\vrule}c|c|c!{\color{black}\vrule}} 
\arrayrulecolor{black}\hline
\textbf{metric} & \textbf{coef} & \textbf{p-val}                                                     & \textbf{metric}     & \textbf{coef} & \textbf{p-val} & \textbf{metric} & \textbf{coef} & \textbf{p-val}                                                        \\ 
\arrayrulecolor[rgb]{0.8,0.8,0.8}\hline
open rate       & -0.038        & 0.768                                                              & log(1+reading time) & -0.007        & 0.542          & relevance rate  & 0.026         & 0.775                                                                 \\ 
\hline
click/read rate & 0.169         & \begin{tabular}[c]{@{}c@{}}0.026*\\CI{[}0.023, 0.315]\end{tabular} & read rate           & 0.027         & 0.811          & click rate      & 0.221         & \begin{tabular}[c]{@{}c@{}}0.049*\\CI{[}0.001, 0.441]\end{tabular}    \\ 
\hline
read speed      & 0.007         & 0.786                                                              & detail rate         & 0.055         & 0.629          & comment rate    & -0.260        & \begin{tabular}[c]{@{}c@{}}0.041*\\CI{[}-0.508, -0.012]\end{tabular}  \\
\arrayrulecolor{black}\hline
\end{tabular}
}
\end{table}

\section{Discussion}
In this paper, we studied how to support communicators in evaluating organizational bulk emails. We conducted expert interviews to understand design requirements. Then with an iterative design approach, we deployed the system CommTool. At last, we evaluated CommTool in a 2-month field test with 149 employees and 5 communicators.

We found that communicators wanted more details like message-level metrics to help them better evaluate and target bulk messages (RQ1). Employees were paying less and less attention to the tested channels therefore channels' reputation needs to be monitored (RQ2). Communicators used CommTool to better understand their audience and also suggested improvements on features like cost estimation, group-level interest, etc (RQ3). Email's click rate and comment rate are significantly correlated with their channels' reputation (RQ4). In the below, we discussed the observations we found interesting.

\subsection{Influence of Organization Structure on Evaluating Bulk Emails}
We observed that the organization's structure influences communicators' use of bulk email evaluation platforms. In the field test, though communicators had access to the evaluation reports and felt that certain email designs could be changed, they did not always have the final say on whether a message should be sent out and they needed to get back to their clients, the organization leaders. The separation of information access and decision-making brought extra costs for CommTool's users in communicating back and forth with their clients if they would like to make changes. CommTool tried to reduce this cost by enabling communicators to share reports with their clients. However, this approach does not significantly influence leaders' decisions. Communicators suggested that leaders would need the reports to be more appealing: 

\textit{``If that (the report) was going to be used to show your leadership, it might provide something easier to prepare, more appealing, like a presentation'' (P5)}. 

Another high-level solution to this challenge is to transfer part of the decision power to communicators. As \citeauthor{jensen2009specific} proposed in their paper about organization's knowledge control and structure \cite{jensen2009specific}, \textit{``If the knowledge valuable to a particular decision is to be used in making that decision, there must be a system for partitioning out decision rights to individuals who already have the relevant knowledge and abilities or who can acquire or produce them at the lowest cost''}. For example, the organization leaders could allow communicators to remove some messages themselves if the history reports show that those types of messages are not interesting to the audience.



\subsection{Making positive suggestions}
One interesting observation is that communicators found the message-level reading time useful but cost less helpful, while cost is approximately a rephrase of reading time in CommTool. Communicators reflected that the cost displayed is too ``frightening'' to lead them to make any decisions based on that. Intuitively, reading time and cost can be viewed as the positive side and negative side of the same concept. The fact that users are more likely to take actions based on the positive side match with the previous findings on psychology --- for example, \citeauthor{hayashi2012pedagogical} and  \citeauthor{kim2007pedagogical} both found that students/participants were more motivated to learn when they received positive feedback from conversational agents \cite{hayashi2012pedagogical}. This observation suggests that bulk email evaluation platforms could benefit from making the reports' presentation more positive to encourage communicators to take action in designing / targeting.

\subsection{Reputation needs to be measured and protected}
In this study, we found that the reputation of channels was decreasing as recipients were opening fewer emails and reading faster through the field test. This result shows that the reputation of communication channels needs to be monitored as the communication channels could be ineffective in delivering information. In our experiment, the read rate decreased by over 30\% as recipients gradually learned to stop reading some channels. 

A challenge of monitoring reputation is to give it a good definition. Actually, the field test found that communicators did not like to use the ``reputation'' which is defined as a specific number --- they preferred to observe the trend of diverse metrics themselves. Therefore reputation needs to be defined or presented more intuitively, for example, the predicted future open rate / read rate of channels. Another challenge is to protect reputation. For example, bulk email evaluation platforms could be combined with personalization platforms to mix the messages that the organization finds important with the messages that the employees like to maintain employees' positive perceptions of those channels \cite{10.1145/3555641}.


\section{Conclusion}
In this paper, we studied how to support communicators evaluating organizational bulk emails to improve organizational communication's effectiveness. We started with expert interviews with 5 communicators. We found that communicators wanted more detailed information like message-level reading time, relevance rates, comments, etc to help them understand their audience. Then with an iterative design approach, we deployed an organizational bulk email evaluation platform CommTool. CommTool gives communicators convenient real-time access to not only email-level but also message-level reading time, read rate, read-in-detail rate, relevance rate, comments, group-level interests, etc. We then conducted a 2-month field test with 5 communicators and 149 employees to evaluate CommTool. We collected employees' interactions through the field test and communicators' feedback through surveys during the field tests, as well as interviews after the test. We found that communicators liked the message-level reading time, read rate, and relevance rate provided by CommTool, which helped them to better understand their audience's interests in each message. Comments helped communicators in designing messages though communicators might be too busy to check all of the comments. Communicators trust the reputation and cost algorithm, but felt that they preferred to observe the trends themselves and use that as reputation instead of a number, and their clients felt that some messages should be sent out at such costs. 

The limitations of this study include that 1) though the tested channels are selected from the newsletters that target the whole organization, their mailing list is not the same as our participant list and the measured metrics would not be the same as these channels' performance on their real mailing list; 2) we conducted our study in a large organization with a top-down communication system; organizations with different structures (such as a flattened management structure) might have different findings (for example, their communicators might have more say in deciding which messages to be sent out).

With these limitations, this study contributes to improving organizational communication by understanding communicators' expectations, and deploying and testing a bulk email evaluation platform with diverse message-level and email-level metrics on awareness, relevance, cost, and reputation. Based on the test, this study suggests bulk email platforms add certain message-level metrics such as reading time and read rate, and gives specific recommendations on how to present these metrics to make them helpful for communicators.








%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.


% \section{Research Methods}
















==> conclusion_backup.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% conclusion.tex:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Discussion and Conclusion}
\label{conclusion_chapter}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this chapter, I summarize the contributions of the previous chapters, the implications of our findings, and future work. By conducting surveys, interviews, controlled field experiments, and iterative design studies, this work brings artifacts on how organizational bulk email system works, and at which control points we can insert interventions to make this system more effective.

\section{Contribution Summary}
We started this thesis from our personal experience with the study site --- why as an employee, we receive hundreds of pieces of non-targeted and non-personalized information from the university through bulk emails every week. In a follow-up meeting with 9 communicators of the study site, we learned that the study site's organizational bulk email system might be ineffective and not what the university wanted it to be. Then we looked back to previous work, and found much knowledge on how organizational communication's effectiveness is impacted by various stakeholders' actions, but less knowledge on organizational bulk emails, especially from a multi-stakeholder perspective. Therefore we identified a need to understand this system's effectiveness and its stakeholders, and to dig into the technology opportunities for making this system better.



In Chapter 4, we first conducted a mixed-methods study to understand organizational bulk email system and its stakeholders. Through a survey of 162 employees of our study site, we learned that the current organizational bulk email system is ineffective as only 22\% of the information communicated was retained by those employees. Then through the artifact walkthroughs with 6 communciators, 9 recipients, and 2 managers, we learned that the failure of the study site's organizational bulk email system was systematic — the organizational bulk email system had many stakeholders, but none of them necessarily had a global view of the system or the impacts of their own actions. The senders would like their messages to be distributed broadly. The communicators lacked tools for personalizing, targeting, and evaluating bulk emails. The employees, overwhelmed by large quantities of information, only want to read messages relevant to themselves. 

In Chapter 5, based on the findings of the empirical study, we further proposed an economic model to describe the value, cost, and actions of this system's stakeholders and how their diverse perspectives cause ineffectiveness. We summarized two promising interventions. On the recipient side, we need mechanisms for incentivizing employees to read high-level information. On the sender side, we need to let senders consider the value and cost of their bulk messages, and design tools for communicators to support them in making targeting and designing decisions. We then conducted two studies corresponding to these two interventions.


In Chapter 6, we studied the recipient-side interventions --- the personalization designs of organizational bulk emails that can lead employees' attention to the messages important to the organization, while maintaining employees' positive experiences with these bulk emails, then they continue to read these emails in the future. In an 8-week field experiment with a university newsletter, we implemented a 4x5x5 factorial design on personalizing subject lines, top news, and message order based on both the employees' and the organization's preferences. We found that mixing important-to-organization messages with employee-preferred messages in top news could improve the whole newsletter's recognition rate. This work also provided a basic backend framework for communicators in personalizing organizational bulk emails.

In Chapters 7 \& 8, we studied the sender-side interventions --- an evaluation tool that supports communicators in making editing and targeting decisions on organizational bulk emails. We iteratively designed and deployed an organizational bulk email evaluation platform (CommTool), which enables communicators to evaluate the message-level metrics and estimate email's impact on channel reputation. We evaluated CommTool through a 2-month field test with 5 communicators and 149 organization employees.
  We found that 1) the message-level metrics such as reading time and read rate helped communicators in designing; 2) email's performance is correlated with its channels' future reputation; 3) CommTool does not influence the organization leaders' decisions. We summarized with suggestions on designing organizational bulk email evaluation platforms that consider leadership and provide positive feedback. At the same time, we built a neural network model that reached a 27\% percentage error in per-message reading time estimation based on user interactions only, against the 200k ground truth data points we collected through eye-tracking tests.

% Then we designed and deployed an organizational bulk email evaluation platform (CommTool). During the deployment, we also built a model and the infrastructure to enable evaluation platforms to estimate per-message reading time and read level solely based on user's interactions with webpages. Specifically, we conducted eye-tracking tests recording participants reading e-newsletters and collected 200k datapoints. We reached 70\% accuracy in reading time estimation with a two-tower neural network model.

% Then we evaluated CommTool. We conducted 7 usability tests, and a 2-month field test with 4 communicators and 151 recipients (employees). We found that 1) the story-level metrics provided by CommTool are useful for communicators in making decisions in editing / targeting; 2) bulk email's performance impacted its venues' reputation.

In short, this thesis provided: 1) the artifacts on how organizational bulk email system works and its stakeholders' perspectives; 2) the mechanisms on how to lead organizational bulk emails' recipients and senders to the actions towards the whole organization's benefit; 3) the personalization tools and evaluation tools to support communicators in better designing and targeting organizational bulk emails. 


\section{Discussion and Future Work \cite{kong_social_agent}}
Based on our studies, we highlighted that organizational bulk email systems should be designed differently from the existing commercial bulk email systems based on their nature as a system in the workplace and for organizations.

\subsection{Design Lessons}


\subsection{Nuances, Fluidity, and Exceptions as a Workplace System}
Like many social technology systems in workplaces, organizational bulk email system is full of nuances, fluidity, and exceptions \cite{ackerman2000intellectual}.

``Nuances'' refers to the depth of details needed for understanding the contexts to make predictions and decisions \cite{ackerman2000intellectual}. All the stakeholders in organizational bulk email system have very nuanced perceptions of the context. For employees, whether they perceive a message as work-relevant depends on their job responsibilities, which can be complicated and obscure. For example, in 4.7.5, we discussed a bulk email reminding Webex users to transfer their documents. Strictly, this information is only relevant to those employees who have not transferred their files and would need to use those files in the future. This granularity of information is hard to collect (especially implicitly without asking employees), and is case-by-case --- emails with different contents would definitely need different context. It is obvious that an effective organizational bulk email system, ultimately, would build on certain knowledge management systems that can identify the required contexts smartly and collect them automatically \cite{maier2011knowledge}. For example, a knowledge management system that stores employees' job responsibilities and preferences to decide which bulk messages are relevant to them.

``Fluidity'' refers to the changes in stakeholders' perspectives and practices  \cite{ackerman2000intellectual}. For example, employees' actions toward bulk emails might depend on their schedules. In Table \ref{tab:disagree}, employee R6 skipped a bulk email because they were too busy that month and found the email relevant when we asked them to read it. Employees' job range is also fluid. Using the ``voicemail down'' message in Chapter 5 as an example, this kind of message might be relevant to an employee if they are planning for a voicemail message on Sunday but might be irrelevant if they have no such plans next time. Also, for the senders, there are less common criteria on how to send a bulk message (see 4.7.2). One communication channel can be used to send important and good-to-know messages at the same time, which would cause employees' confusion about the importance of the messages from that communication channel. Given the fluidity of organizational bulk email system, it is important for the knowledge management system to collect contexts in real time. For example, updating employees' time schedules and controlling the quantities of information they receive according to that.

``Exceptions'' --- the revision of general guidelines in practice --- are normal in workplace \cite{suchman1984procedures}. Indeed, the stakeholders in organizational bulk email systems do not completely follow rational standards. Whether and how a bulk message would be sent not only depends on its objective value, but also the perceptions and level of its senders. For example, in Chapter 5, the message \textit{``UMD Chancellor Search''}, though mainly relevant to a single campus, was sent to the employees across all the campuses as a single email, because the sender perceived the value of their message being distributed widely. Therefore organizational bulk email systems should have back-channels that allow stakeholders to negotiate when an exception can be made and evaluate the impacts of exceptions (e.g., the impact on channel reputation of sending a good-to-know message to all the employees).

\subsection{Stakeholders with Different Goals and Perspectives in Organizations}
Besides nuances, fluidity, and exceptions, stakeholders' perceptions might also exist conflicts that pose challenges to the decision process of organizaitonal bulk email system. The information producers (like organization leaders) value that their messages be heard widely; the communicators would like to meet their clients’ requirements with minimal time and effort; the employees would like to get the information they perceive as useful themselves efficiently. In commercial bulk email systems, we can focus on one single stakeholder's perspective, like helping recipients filter bulk emails or helping senders improve their open rate. However, in organizational bulk email systems, stakeholders have the responsibility of considering others'  and the whole organizations' value. 
However, in the current system, none of the stakeholders would be able to see the impact of their actions on the whole organization. Therefore we need to design tools to provide stakeholders access to such impact and mechanisms that can incentivize stakeholders to act toward the whole organization's benefits.

To enable such visibility, in this thesis, we designed one personalization tool that incentivizes employees to read important messages (Chapter 6) and one evaluation tool that enables senders to understand the performance and cost of the bulk messages they send (Chapters 7 \& 8). But visibility might not be enough to influence the dynamics of the current system, because there are exceptions (e.g., some senders' strong willingness to get their messages out). Indeed, an important question to be studied is who has the final say on whether a message should be sent via a channel. We can think about three approaches here. The first approach is to use an agent. For example, we can make decisions based on the economic model in Chapter 5, and a bulk message can only be sent out when its predicted return is positive. If we follow this direction, we will need to build more complete models to predict employees, communicators, and leaders' perceptions of or actions on bulk emails. These would include studies on predicting open rates, reading time, interest rates, etc. Then we connect all these elements together to predict the whole organization's value and cost with bulk communication. The second approach is to let stakeholders make their own decisions based on the system's expectations. For example, an organization can allocate communication budgets to units to reduce wasteful or poorly-targeted organizational bulk emails. The third practical approach is to enable some negotiation mechanisms between stakeholders \cite{strauss2018creating} when conflicts happen. For example, giving recipients the access to unsubscribe from certain messages while still receiving important ones; enabling communicators to discuss how each communication channel should be used, and scheduling messages unitedly.

But even without these steps, we believe that the visibility tools in this thesis could provide the incentive to already well-motivated communicators.

\subsection{From Science to Engineering}
With all these nuances, fluidity, exceptions, and conflicts, it is noticeable that there will be a gap between science and engineering in designing organizational bulk email systems. A significant problem is the quantifying of message value. We discussed various stakeholders' value in Table \ref{tab:cost_summary}, such as the information producer's value of their message being heard, the evidence of getting the information out, etc. However, to plug these value into the calculation of decision mechanisms of bulk emails (the return formulas in Table \ref{tab:cost_summary}), we need different stakeholders' value, cost, and reputation to be comparable. And even a simple question like turning the value of ``the relevant employees know what the senders are trying to disseminate'' into some quantifiable scale, like money, would be an interesting problem for management and economics studies. In Chapter 6, we use participants' ratings to quantify messages' value but do not compare the value with cost. In Chapters 7 \& 8, we just show all the value and cost without transforming them into the same scale. In short, there is much work to be done to turn what we learned from this thesis into what we can design in engineering without loss of information.

In short, with this thesis, we now understand organizational bulk email systems' stakeholders' value, and how personalization and visibility tools could be used to influence employees' and senders' behavior toward the whole organization's benefits. And give the nuances, fluidity, exceptions, and conflicts in organizational bulk email system, there is still work to be done to manage this system's knowledge, quantify its metrics, and make decisions on designing / targeting bulk emails.


% At last, on the topic of organizational bulk email systems, I would like to highlight the necessity of collaboration between academia and industry. To build complete models to predict the stakeholders' actions and perceptions, the amount of data we need would be much larger than the current work email datasets like Avocado \cite{yang2017characterizing}, Enron Corpora \cite{bekkerman2004automatic}, because each datapoint we need would be a complex of the datapoints of many employees, messages, and channels. To gather such an amount of data, we would need to embed the data collection process into the current business platforms.



==> current_results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% current_results.tex: {{{
% Chapter on neutrino oscillation experiments and current result.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Current Neutrino Oscillation Experimental Results}
\label{current_results_chapter}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Solar neutrino experiments {{{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Solar Neutrinos}

\subsection{Homestake}

\subsection{SAGE and Gallex}

\subsection{SNO}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Reactor neutrino experiments {{{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Reactor Neutrinos}

\subsection{CHOOZ}

\subsection{KamLAND}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Atmospheric neutrino experiments {{{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Atmospheric Neutrinos}

\subsection{IMB}

\subsection{Super-K}

\subsection{MACRO}

\subsection{Soudan 2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Accelerator neutrino experiments {{{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Accelerator Neutrinos}

\subsection{Nomad}

\subsection{LSND}

\subsection{MiniBooNE}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%}}}


==> discussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% event_selection.tex: Select of showering and tracking events:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Discussion}
In this chapter, we discuss the implications of our findings and summarize the potential directions for improving the organizational bulk email system. From the perspectives of different stakeholders, we should further explore how to improve employees' awareness of the bulk messages important-to-organization, encourage communicators to consider employees' burden, and raise organization's awareness of the relative performance and cost of bulk email communication. From the perspectives of study areas, there are three major fields to work on --- models, tools, and mechanisms. We could first build models to predict stakeholders' perceptions and actions with organizational bulk emails; then design mechanisms that utilize the models to incentivize the stakeholders to take effective actions; lastly, incorporate the incentives into practical tools.



% \begin{table}
% \centering
% \caption{The potential research directions in organizational bulk email systems given the perspectives of stakeholders and research fields.}
% \label{tab:direction}
% \begin{tabular}{|l|l|l|l|} 
% \hline
% \textbf{User\textbackslash{}Field}                                               & \textbf{Models}                                                                                                                                                       & \textbf{Tools}                                                                                                                                                                                                                                                                                                                                                                       & \textbf{Mechanisms}                                                                                                                                                                                                                                                                                               \\ 
% \hline
% \textbf{Employees}                                                               & \begin{tabular}[c]{@{}l@{}}Predict employee's \\\textcolor{blue}{perceptions of (study 2)}\\/actions with bulk emails. \\\end{tabular}                                & \begin{tabular}[c]{@{}l@{}}\textbf{\textbf{Increase Value}}\\Support employees in \\filtering irrelevant bulk \\emails.\end{tabular}                                                                                                                                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}\textcolor{blue}{\textbf{\textbf{\textbf{\textbf{Increase Value}}}}}\\\textcolor{blue}{Incentivize employees to read}\\\textcolor{blue}{the important-to-organization}\\\textcolor{blue}{messages. (study 2)}\end{tabular}                                                             \\ 
% \hline
% \textbf{Communicators}                                                           & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Predict sender's perceptions\\of bulk emails' value.\end{tabular}}                                                         & \begin{tabular}[c]{@{}l@{}}Support communicators in\\\textcolor{blue}{\textbf{(Increase Value)}}\\\textcolor{blue}{\textbf{personalizing~}(study 2),} \\targeting\\\textcolor{red}{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{\textbf{(Limit Cost)}}}}}}}}}\textbf{\textcolor{red}{evaluating~}}\textcolor{red}{bulk emails }\\\textcolor{red}{(study 3)}.\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{\textbf{\textbf{\textbf{Limit Cost}}}}\\Incentivize communicators\\to~consider~whether~bulk\\messages~should be sent\\based on the value,\\\textcolor{red}{performance,~ cost, reputation}\\\textcolor{red}{of bulk communication. }\\\textcolor{red}{(study 3)}\end{tabular}  \\ 
% \cline{1-1}\cline{3-4}
% \begin{tabular}[c]{@{}l@{}}\textbf{Organization }\\\textbf{Leaders}\end{tabular} &                                                                                                                                                                       & \begin{tabular}[c]{@{}l@{}}\textbf{Limit Cost}\\Support leaders in \\allocating the budgets of \\bulk communication.\end{tabular}                                                                                                                                                                                                                                                    & \begin{tabular}[c]{@{}l@{}}\textbf{\textbf{Limit Cost}}\\Incentivize leaders to \\consider whether bulk \\messages should be sent.\end{tabular}                                                                                                                                                                   \\ 
% \hline
% \textbf{Organization}                                                            & \begin{tabular}[c]{@{}l@{}}Predict bulk email's impact\\on organization's value,\\cost, \textcolor{red}{channel reputation}\\\textcolor{red}{(study 3).}\end{tabular} & \textbackslash{}                                                                                                                                                                                                                                                                                                                                                                     & \textbackslash{}                                                                                                                                                                                                                                                                                                  \\
% \hline
% \end{tabular}
% \end{table}


It could be seen that there are many studies left to be done in organizational bulk email systems. First, we could try to build more complete models to predict employees, communicators, and leaders' perceptions of or actions on bulk emails. These would include studies on predicting open rates, reading time, interest rates, etc. Then by the economic model proposed in chapter 5, we could connect all these elements together to predict the whole organization's value and cost with bulk communication. Second, besides evaluation tools, we could develop other tools to support communicators in targeting and designing bulk emails after we have complete models for predicting employees' actions and perceptions. At an extreme, an organization might even allocate communication budgets to units to reduce wasteful or poorly-targeted organizational bulk emails, but even without this step, we believe the visibility of performance/cost could provide incentive to already well-motivated communicators.  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> paper_attachment.tex <==
\chapter{Papers}
\label{paper_attachment}
\section{Organizational Bulk Email System}
\textbf{Chapter 4:} Ruoyan Kong, Haiyi Zhu, and Joseph A. Konstan. 2021. Learning to Ignore: A Case Study of Organization-Wide Bulk Email Effectiveness. Proc. ACM Hum.-Comput. Interact. 5, CSCW1, Article 80 (April 2021), 23 pages. (completed)

\noindent\url{https://dl.acm.org/doi/10.1145/3449154}

\noindent \textbf{Chapter 5:} The Challenge of Organizational Bulk Email Systems: Models and Empirical Studies (under review for Elgar Information Economics)

\noindent\url{https://drive.google.com/file/d/1Es29SETiDjWGoDX5yRv3GRi_HuaKabQT/view?usp=sharing}

\noindent \textbf{Chapter 6:} Ruoyan Kong, Charles Chuankai Zhang, Ruixuan Sun, Joseph A. Konstan. Multi-Objective Personalization in Multi-Stakeholder Organizational Bulk E-mail: A Field Experiment. (under review for CSCW)

\noindent\url{https://drive.google.com/file/d/1_0OscwA9c35l72OrfrgaQpdjvpUtqisd/view?usp=sharing}



\noindent Ruoyan Kong, Haiyi Zhu, and Joseph Konstan. 2020. Organizational Bulk Email Systems: Their Role and Performance in Remote Work. The New Future of Work. 2020. \url{https://www.microsoft.com/en-us/research/uploads/prod/2020/07/NFW-Kong-et-al.pdf}

\section{Others}
\subsection{Conference Papers}
\noindent Zhang, Charles Chuankai, Mo Houtti, C. Estelle Smith, Ruoyan Kong, and Loren Terveen. "Working for the Invisible Machines or Pumping Information into an Empty Void? An Exploration of Wikidata Contributors' Motivations." Proceedings of the ACM on Human-Computer Interaction 6, no. CSCW1 (2022): 1-21.

\subsection{Workshop Papers}
\noindent Ruoyan Kong, Zhanlong Qiu, Yang Liu, and Qi Zhao. "NimbleLearn: A Scalable and Fast Batch-mode Active Learning Approach." In 2021 International Conference on Data Mining Workshops (ICDMW), pp. 350-359. IEEE, 2021.

\noindent\url{https://ieeexplore.ieee.org/document/9679963}

\noindent Ruoyan Kong, Ruobing Wang and Zitao Shen, Virtual Reality System for Invasive Therapy, 2021 IEEE Conference on Virtual Reality and 3D User Interfaces Abstracts and Workshops (VRW), 2021, doi: 10.1109/VRW52623.2021.00227.

\noindent\url{https://ieeexplore.ieee.org/document/9419157}

\subsection{Under-Review Papers}
\noindent Ruoyan Kong, Ashlee Milton, Daniel Kluver, Ruixuan Sun, Ian Paterson, Joseph A. Konstan. A Case Study of a Recommendation Website's Productive Flyby Users. (under review for Recsys 2022)
~\\

\noindent Ruixuan Sun, Ruoyan Kong, Qiao Jin, Joseph A. Konstan. Less Can Be More: Exploring Population Rating Dispositions with Partitioned Models in Recommender Systems. (under review for Recsys 2022)
~\\

\noindent Yunzhong He, Cong Zhang, Ruoyan Kong, Chaitanya Kulkarni, Qing Liu, Ashish Gandhe,
Amit Nithianandan, Arul Prakash, Query Categorization at Facebook Marketplace: An End-to-end Approach. (under review for SIGKDD 2022)

\subsection{In Preparation}
\noindent Guy Aridor, Duarte Goncalves, Daniel Kluver,Ruoyan Kong, Joseph A. Konstan. The Value of Recommender Systems:
Decomposing the Informational and Discovery Gains (In preparation)







==> study_site.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% simulation.tex: Chapter on MC production:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Study Context}
\label{study_site}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Study Site and Its Organization Structure around Bulk Emails}
We carried out our studies at the University of Minnesota, a large university with approximately 24,000 employees and five campuses. We met with a group of 9 communicators within this university at the beginning of this project. In the meeting, we found agreement that the current bulk email system was not what the university wants it to be, since the communicators felt that bulk emails were ignored too often. They encouraged us to move forward. 

Figure \ref{fig:bulk_structure} is the structure of the organizational bulk email system. Like many large universities, it has both centralized and decentralized governing structures. Each major unit has a communication office or communicators (communication director/staff). There are central units led by university leaders responsible for the core business functions. The University Relations office (under the Vice President for University Relations) is in charge of internal communications for the university. Each Vice President’s office has a communication unit or several communication staff, who draft and send emails for university leaders and conduct university-wide bulk email communications through newsletters. Many central units run their own newsletters. Employees are subscribed to many of these newsletters by default. 

The non-central units like colleges' Deans’ offices also perform bulk communications locally. Their communicators conduct local communications and also work with central communication offices, such as collecting and submitting content to the central newsletter editors, or redistributing the messages from the central units.  

The IT infrastructure provides technical support for the bulk email system, including an email system (Gmail), an email marketing platform (Salesforce), and a human resource system (Peoplesoft). The email marketing platform controls the access to sending bulk emails to campus-wide groups via mailing lists or query-based databases. Only trained communicators have access to the corresponding authorized mailing lists. It is worth noting that querying the exact group of employees can often be difficult and time-consuming. For example, there is no clear definition of ``researchers'' in the PeopleSoft database. To send a message to all the ``researchers'' of the university, the communicators need to read the definitions of hundreds of job codes to judge whether each job code should be included in the mailing list.

\begin{figure}[!htbp]
\centering
  \includegraphics[width=1\columnwidth]{study1_folder/bulk_structure.png}
  \caption{Organization structure of the University of Minnesota related to bulk communication; ``SVP'', ``EVP'', ``VP'': (Senior/Executive) Vice President’s offices; “comm”: communication units or communicators. Details of other campuses and many central units are not shown. Some units also conduct external bulk communication (e.g., emails to alumni and the general public), which is not shown here.}~\label{fig:bulk_structure}
\end{figure}





